Recent Progress in the Theory of Bulk Photovoltaic Effect

The bulk photovoltaic effect (BPVE) occurs in solids with broken inversion symmetry and refers to DC current generation due to uniform illumination, without the need of heterostructures or interfaces, a feature that is distinct from the traditional photovoltaic effect. Its existence has been demonstrated almost 50 years ago, but predictive theories only appeared in the last ten years, allowing for the identification of different mechanisms and the determination of their relative importance in real materials. It is now generally accepted that there is an intrinsic mechanism that is insensitive to scattering, called shift current, where first-principles calculations can now give highly accurate predictions. Another important but more extrinsic mechanism, called ballistic current, is also attracting a lot of attention, but due to the complicated scattering processes, its numerical calculation for real materials is only made possible quite recently. In addition, an intrinsic ballistic current, usually referred to as injection current, will appear under circularly-polarized light and has wide application in experiments. In this article, experiments that are pertinent to the theory development are reviewed, and a significant portion is devoted to discussing the recent progress in the theories of BPVE and their numerical implementations. As a demonstration of the capability of the newly developed theories, a brief review of the materials design strategies enabled by the theory development is given. Finally, remaining questions in the BPVE field and possible future directions are discussed to inspire further investigations.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
